What's in a Caption? Dataset-Specific Linguistic Diversity and Its Effect on Visual Description Models and Metrics

While there have been significant gains in the field of automated video description, the generalization performance of automated description models to novel domains remains a major barrier to using these systems in the real world. Most visual description methods are known to capture and exploit patterns in the training data leading to evaluation metric increases, but what are those patterns? In this work, we examine several popular visual description datasets, and capture, analyze, and understand the dataset-specific linguistic patterns that models exploit but do not generalize to new domains. At the token level, sample level, and dataset level, we find that caption diversity is a major driving factor behind the generation of generic and uninformative captions. We further show that state-of-the-art models even outperform held-out ground truth captions on modern metrics, and that this effect is an artifact of linguistic diversity in datasets. Understanding this linguistic diversity is key to building strong captioning models, we recommend several methods and approaches for maintaining diversity in the collection of new data, and dealing with the consequences of limited diversity when using current models and metrics.

==> sec/Z_3_method.tex <==
\section{Background \& Related Work}










% \paragraph{Conceptual Captions} Conceptual Captions is a large-scale dataset for image captioning, containing 3.3 Million images, and their associated captions sourced from Alt-Text on the internet. While the captions are automatically sourced, there are several filtering steps which aim to reduce non-descriptive text.


% \subsection{Baseline Models}

% In some cases, we use a baseline auto-regressive model for video captioning, trained on the MSR-VTT dataset, to explore claims about caption diversity and generation. The full details of this model are presented in the supplementary materials, and code is made available at \verb|public URL|. 

% \paragraph{S-MiT} The S-MiT dataset \CN (Spoken Moments in Time) is a large-scale open domain video description benchmark, based on the Moments in Time dataset. The S-MiT dataset collects gold-standard audio recordings of a person describing each of 515,912 short 3-second video clips. These audio clips are then transcribed to natural language with Google's automated speech recognition toolkit. 

% \paragraph{Charades} The Charades \CN dataset contains 9848 videos of daily indoor household activies, recorded by 267 Amazon Mechanical Turk users (all of whom followed a script to produce a video clip). The videos average 30 seconds each, and cover 157 unique types of actions, and 46 objects. 
 
% \paragraph{ActivityNet Captions}The ActivityNet captions dataset \CN is a medium-scale open domain video description benchmark drawn from the ActivityNet database dataset. It covers 200 classes, with 20,000 videos. For each video, 5 clips are taken (each approximately 36 seconds of video), and annotated with a single action description. 

% \paragraph{YouCook-2} The YouCook-2 dataset \CN is a small-scale cooking-domain video description benchmark which contains 2000 videos uniformly distributed over 89 recipes. The videos are sourced from YouTube, and divided into 3-16 segments each, with an average of 7.7 segments per video (each segment ranging from 1 to 264 seconds). 

==> sec/Z_4_results.tex <==
\section{Motivation}
\label{sec:motivation}




% \subsection{Discussion}

% In the previous sections, we have analyzed the concept of linguistic diversity across several axes, which lead us to the hypothesis \textbf{H1: Metrics are influenced heavily by the number, and diversity of available ground truths, leading to models which exploit trends in the most common ground truth samples}. The above experiments provide ample support for this observation. As we saw in \autoref{sec:tld}, at a token level, these visual description datasets have a very long tail, and the length of this tail is directly related to downstream metric performance: a longer tail means less reliance on tail tokens in the metric scores. At an n-gram level, we demonstrated in \autoref{sec:ngld} that most visual description datasets rely on making very few choices during the generative process, which we hypothesize is a major contributor to bland/generic test-time captions. At the dataset level, in \autoref{sec:dld} we show that the metrics are subtly influenced by even the number of ground truth captions collected.  





\subsection{H3: Regression of Models to the Worst Captions}
\label{sec:h3}

There are two unique levels of diversity that need to be maintained when collecting a dataset. In \autoref{sec:h1}, we explored diversity primarily at a sample level. This kind of diversity is controlled during the labeling phase of the dataset collection, and additional diversity can be induced by differing techniques for labeling. In addition to sample level diversity, we also need to think about how the choice of samples impacts the dataset, a choice that is made when choosing which samples to label, and is usually selected by the dataset authors. The impact of poor sample diversity is dual with labeling diversity: If visual samples are not diverse, then to avoid generating generic descriptions at test time, the sample-level labels must be even more diverse. If the visual samples are very diverse, the label diversity can afford to be more coarse, as a wider range of subjects and scenes are depicted, and while the descriptions may live at a higher semantic label, the model is more likely to learn to diversely describe the dataset. This lack of both visual diversity and sample-level diversity together leads to a unique kind of model: a model which focuses on classification over generation, and can reproduce descriptions from the training set which are generic, yet often semantically correct. 


From \autoref{sec:coreset} and \autoref{sec:fsi}, we can see that the current visual datasets are extremely vulnerable to inducing classification over generation in downstream models, supporting our hypotheis: \textbf{(H2): Models can exploit a ``classification" vs ``generation" effect, where it is sufficient to understand only a small amount of information about a sample in order to generate captions which are likely to match at least one ground truth sample.}

 While we have not shown that this happens in practice, we have demonstrated that models may be able to achieve strong performance by sticking to common dataset captions, and only focusing on large-scale ideas. This bias towards classification leads to captions that are approximately correct, however do not contain a sufficient level of detail for visually impaired users \cite{hendricks2018women, macleod2017understanding}. 

\TODO{Additional Discussion here}











% \section{Analyses and Discussion}

% The primary goal of this paper is to build a more complete picture of the current benchmarks for visual description, and quantify many of the difficulties that researchers face when developing generalizable visual description methods. We explore in detail several facets of video description datasets, and compare and contrast the details of the datasets with the current SOTA performance on these datasets in the field, to demonstrate connections between the design of the dataset, and the quality of the models.

% \subsection{Are ``Gold-Standard captions" really golden?}

% \subsubsection{Oracle Human Performance}

% Several of the datasets that we explore collect several ground truth samples, which begs the question: how well do ground truth samples perform on the given datasets? To test the performance of the colelcted ground truths, for each video we sampled a single ground truth to test, and computed the standard video description metrics with respect to the other ground truths as a baseline. We repeat the sampling process over the full dataset 750 times, to get a good estimate of the distribution of the data. The results of this experiment are presented in Table \TODO{GT Distribution Table}. While the ground truths do perform well (and much better than some early methods), we also find that in all of the datasets with multiple ground truth samples, current SOTA captioning methods are outperforming the ground truth samples on the standard metrics. With further review, we found the captions represent a diverse, and traditionally non-expert set of descriptions. Thus, captions can focus on a myriad of likely subjects, with various levels of detail, leading to a large number of ground truth captions required to saturate the full space of ideas. 

% \subsubsection{Baseline Performance}

% We believe that in the case of conditional modeling datasets, it is important to have an understanding of a set of baseline performance numbers for each of the datasets. Table \TODO{table:baselines} presents the baseline scores of several simple models (details in the supplementary materials). From this, we can see that while the baseline models are under-performing the SOTA models (as we would hope), there are a number of published works, particularly in the zero-shot domain which do not outperform simple baselines. Using the baseline models, we introduce a ``hard-mode" split of the test datasets, which isolates samples with low likelihood under general language models. We can see that our baseline model has significantly reduced performance on this split, while the oracle performance remains stable, suggesting that current models may be heavily biased towards generating simple captions, which focus on exploiting the likelihood of the model. 


% \subsection{Is ``Open Domain" really open?}

% A common figure in several of the descriptions of the datasets is the first two columns Table \TODO{tab:vocab} which demonstrates the linguistic diversity in each of these datasets through the number of tokens in each vocab, and the number of total words in the dataset. While these metrics provide a rudimentary understanding of the linguistic diversity of the dataset - when building models for generalizable visual description, we want to get a fuller picture of the kinds of captions present in the data. 

% \subsubsection{Token-Level Diversity}

% One of the common complaints of many visual description methods is that the models regress to simple utterances with little detail, such as ``a woman is running", as opposed to providing a more complete natural composition. In \CN, the authors proposed several methods for caption evaluation: \textit{uniqueness}, \textit{novelty} and \textit{vocab coverage}. Table \TODO{UNV Table} shows the ground truth values of these metrics for each of the explored datasets, along with reported values for state of the art methods (if they are available). We can see that in many cases, the model values far exceed the values of the ground truths. This experiment once again draws attention to the risk of directly optimizing these metrics as a proxy for caption diversity.

% \subsubsection{N-Gram Complexity}

% Table \todo{N-Gram LM table} presents some of the most common starting n-grams, and their associated likelihoods under an N-gram model. We can see that in some datasets, particular N-grams dominate the likelihood. This effect translates directly to captioning methods. For these N-Grams, a vast majority of captions start with one of these most-common starting pairs. While not a fundamental issue with the modeling process, the overwhelming data bias tends to lead to poor downstream performancs, as demonstrated in \CN. Exploring ways to de-bias the generative process from these starting n-grams will lead to significantly improved performance. Further, we can see that the diversity of the dataset is heavily dependent on the types of n-grams present in the data. Table \TODO{tab:n-gram perplexity} shows the perplexity of an N-gram language model on each of the caption datasets (additional information in the supplementary materials). We can see that while, as a whole, the caption set may be relatively unique, there are a significant number of linguistic patterns that can be captured and exploited for optimal performance. 

% \subsubsection{Caption-Level Diversity}

% In addition to understanding the linguistic diversity at the token and n-gram level, we also want to understand the diversity of the captions in the data. Table \TODO{tab:caption diversity} introduces several metrics for understanding the diversity of captions. 

% \TODO{Unique captions}
% \TODO{Distribution of caption lengths}

% \subsubsection{Conceptual Diversity}

% We also wanted to explore how diverse these different datasets are at a conceptual level. To do this, we present several experiments using automated part-of-speech tagging (POS tagging) \CN, to explore the kinds of words present in the captions. 

% Many video description methods rely on pre-trained models to extract visual features. Perhaps the most common pre-trained models are trained using features from the Kinetics \CN dataset, which depicts between 400 and 700 different types of actions, or from the Imagenet \CN dataset, which focuses on 1K unique image classes. To test if these are appropriate pre-training datasets for the visual description task, we used a combination of verb-stemming and fuzzy matchting to compute the overlap between the Kinetics-600 label set, and the verbs in the visual description datasets, as well as the overlap between the ImageNet label set, and the noun set in the visual description datasets (More details are given in the supplementary materials). Table \TODO{matching table} summarizes the results. Overall, we found that most datasets have between a 10\% and 30\% overlap with the label sets, which represents a weak correlation with the data, but suggests that there is significant room for growth. To see if the overlap correlated with model performance, we generated a test split for the MSR-VTT dataset which contained overlap samples, and non-overlapping samples. Table \TODO{matching performance} summarizes the results. Perhaps unsurprisingly, models trained with the corresponding feature sets perform significantly better (in some cases, several times better) on N-Gram metrics. From the experiment, it is clear that the work in \CN is critical: we must diversify our features in order to achieve more equitable performance across the classes.

% \TODO{Distribution of nouns per caption}
% \TODO{Distribution of verbs per caption}
% \TODO{Distribution of named entities, baseline split for named entities}

% \subsection{How many ground truths are enough?}

% Most of the datasets that we explore have more than one ground truth caption, however it can be extremely expensive to collect additional ground truth captions for a dataset. In this section, we explore the effects that varying the number of ground truth captions can have on the down-stream evaluation of the datasets.

% \subsubsection{What happens when we add more truth?}

% How many ground truth captions does a good benchmark need? Figure \TODO{GTs over time table} shows the experiment from \TODO{sec: before} which simulates ground-truth performance using the common captioning metrics, however we restricted the number of ground truths at each time step. While most metrics tend to increase (or even saturate) as the number of ground truths increases, the CIDEr score has a remarkably different behavior. Because of the tf-idf component in CIDEr, the model is far more likely to penalize common n-grams as the number of ground truths increases. 

% \subsubsection{Generate or Discriminate?}

% A common criticism of captioning models is that they are not generative, but instead reproduce captions from the training set based on a set of global criteria. To evaluate this claim, we explore the oracle performance of several zero-shot techniques, to see if recall-based captioning is viable, and if so, how current generative models perform compared to such recall-based methods. Figure \TODO{base performance} demonstrates the performance of an oracle model selecting the best caption among the top-k most common captions in the training dataset for the visual description datasets, along with the current SOTA models. We can see from this figure that for a number of datasets, our models perform identically to selecting the best caption from  among the top \TODO{numbers} captions. This begs an additional question: if we simulate the performance of a classifier at each point, how well does it perform? Figure \todo{Fig} shows that if we simulate \TODO{num} percent accuracy in a top-k classifier, we can achieve strong performance.


% % \subsubsection{Generative models leave a lot on the table}

% % Figure \TODO{fig} shows that while our captioning models may be regressing to the mean of the most common captions, not all hope is lost for good caption quality. We can see that using an oracle model to re-rank the captions generated by a depth-4 beam search, we can outperform most SOTA models by a wide margin. Selecting from the top 16 captions is even better. Note, that Figure \TODO{fig} shows that it's not the case that there are 16 oracle captions that perform well across the dataset, and instead, the captioning models are just not able to overcome priors in the language data.

% % \TODO{Understanding generation from a lingistic structure perspective}
% % \TODO{Understanding generation from a search perspective, number of beams, etc.}


% \section{Visual Description Dataset Analysis Toolkit}

% 

==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}
